Approximate Denial Constraints

The problem of mining integrity constraints from data has been extensively studied over the past two decades for commonly used types of constraints including the classic Functional Dependencies (FDs) and the more general Denial Constraints (DCs). In this paper, we investigate the problem of mining approximate DCs (i.e., DCs that are "almost" satisfied) from data. Considering approximate constraints allows us to discover more accurate constraints in inconsistent databases, detect rules that are generally correct but may have a few exceptions, as well as avoid overfitting and obtain more general and less contrived constraints. We introduce the algorithm ADCMiner for mining approximate DCs. An important feature of this algorithm is that it does not assume any specific definition of an approximate DC, but takes the semantics as input. Since there is more than one way to define an approximate DC and different definitions may produce very different results, we do not focus on one definition, but rather on a general family of approximation functions that satisfies some natural axioms defined in this paper and captures commonly used definitions of approximate constraints. We also show how our algorithm can be combined with sampling to return results with high accuracy while significantly reducing the running time.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

==> approx_copy.tex <==
\section{Approximate Hitting Sets}
In this section we discuss the relationship between our problem and the \e{minimal hitting set} problem, and provide some definitions that we will later use in our mining algorithm. We first recall some definitions and results given by Chu et al.~\cite{DBLP:journals/pvldb/ChuIP13}. Let $\signature$ be a schema and let $I$ be an instance of $\signature$. Given a pair $\langle t_1,t_2\rangle$ of tuples from $I$, the \e{satisfied predicates set} for $\langle t_1,t_2\rangle$ is 
\[SAT(\langle t_1,t_2\rangle)=\set{P\mid P\in\pspace,\set{t_1,t_2}\models P}\]
That is, $SAT(\langle t_1,t_2\rangle)$ contains all the predicates that are satisfied by $\langle t_1,t_2\rangle$. Then, the \e{evidence set} of $I$ is defined as follows. 
\[Evi_I=\set{SAT(\langle t_1,t_2\rangle)\mid t_1,t_2\in I}\]
Note that two distinct pairs of tuples $\langle t_1,t_2\rangle$ and $\langle t_3,t_4\rangle$ may satisfy $SAT(\langle t_1,t_2\rangle)=SAT(\langle t_3,t_4\rangle)$. In our definitions we assume that $Evi_I$ contains a set of predicates for each pair of tuples in $I$, and the number of occurrences of each set is very important to us, thus we treat $Evi_I$ as a \e{bag} rather than a set; thus, we slightly abuse the notation of a minimal hitting set and use it for bags.
Chu et al.~\cite{DBLP:journals/pvldb/ChuIP13} proved the following.

\begin{citedtheorem}{DBLP:journals/pvldb/ChuIP13}\label{thm:reduction-to-hit}
Let $\signature$ be a schema and let $I$ be an instance of $\signature$. Then, $\forall t_1,t_2 \neg(\overline{P_1}\wedge\dots\wedge \overline{P_n})$ is a valid minimal DC w.r.t. $I$ if and only if $\set{P_1,\dots,P_n}$ is a minimal hitting set for $Evi_I$.
\end{citedtheorem}

%{
%\begin{algseries}{t}{\label{alg:fastdc} An algorithm for enumerating minimal valid DCs}
%\begin{insidealg}{FASTDC}{$I,\signature$}
%\STATE $\pspace=\algname{GeneratePredicates}(I,\signature)$ 
%\STATE $Evi_I=\algname{BuildEvidenceSet}(I,P)$ 
%\STATE $MHS=\algname{SearchMinimalCovers}(I,Evi_I,\emptyset,>_{init},\emptyset)$
%\FORALL {$S\in MHS$}
%\STATE $\Sigma = \Sigma \cup \set{\forall t_1,t_2 \neg(\overline{S})}$
%\ENDFOR
%\FORALL {$\phi\in \Sigma$}
%\IF {$(\Sigma\setminus\set{\phi})\models \phi$}
%\STATE $\Sigma = \Sigma\setminus\set{\phi}$
%\ENDIF
%\ENDFOR
%\end{insidealg}
%\end{algseries}
%}

Recall that the \e{hitting set} problem is the following: given a finite set $K$ and a family $M$ of subsets of $K$, find all the subsets of $K$ that intersect every one of the sets in $M$. A subset $F$ is a \e{minimal} hitting set if no proper subset of $F$ is a hitting set of $M$. In order to generate all the valid minimal DCs, Chu et al.~\cite{DBLP:journals/pvldb/ChuIP13} first build the evidence set $Evi_I$ and then generate all the minimal hitting sets for $Evi_I$. To generate all the minimal hitting sets, they use their own algorithm. In order to generate the approximate DCs, they modify this algorithm to generate approximate hitting sets instead. Since Chu et al.~\cite{DBLP:journals/pvldb/ChuIP13} only considered $m_1^\epsilon$-approximate DCs (that is, DCs that are violated by at most $\epsilon$ of the tuple pairs for some $\epsilon>0$), they defined an approximate hitting set ($\epsilon$-minimal hitting set) as a set that has an empty intersection with at most $\epsilon$ of the subsets. This definition is also used in other works that consider approximate hitting sets in other domains~\cite{VINTERBO2000123, Rioult2010}. We refer to this definition of approximate hitting sets as $m_1^\epsilon$-minimal hitting set to avoid confusion. We now give the formal definition.

\begin{definition}[$m_1^\epsilon$-minimal hitting set]
A set of predicates $S$ is a $m_1^\epsilon$-minimal hitting set of $Evi_I$ if $S$ has an empty intersection with at most $\epsilon$ of the sets in $Evi_I$.
\end{definition}

In this work, we replace the algorithm proposed by Chu et al.~\cite{DBLP:journals/pvldb/ChuIP13} for generating approximate hitting sets by another algorithm and show that it significantly improves the performance. To use this algorithm, we first have to define an approximate hitting set for the rest of the definitions of approximate DCs. We now give the rest of the definitions.

\begin{definition}[$m_2^\epsilon$-minimal hitting set]
A set of predicates $S$ is a $m_2^\epsilon$-minimal hitting set of $Evi_I$ if $S$ has an empty intersection with at most $\epsilon$ of the sets in $Evi_I$ that contain at least $\alpha$ of the predicates from $\overline{S}$.
\end{definition}

\begin{definition}[$m_3^\epsilon$-minimal hitting set]
A set of predicates $S$ is a $m_3^\epsilon$-minimal hitting set for $Evi_I$ if the following holds for at most $\epsilon$ of the tuples $t_j\in I$: there exists a tuple $t_k\in I$ such that $SAT(\langle t_j,t_k\rangle)\cap S=\emptyset$ or $SAT(\langle t_k,t_j\rangle)\cap S=\emptyset$.
\end{definition}

\begin{definition}[$m_4^\epsilon$-minimal hitting set]
A set of predicates $S$  is a $m_4^\epsilon$-minimal hitting set of $Evi_I$ if there exists a subinstance $J$ of $I$ such that $|I\setminus J|<\epsilon|I|$ and $S$ is a minimal hitting set of $Evi_J$.
\end{definition}

For each one of these four definitions we denote by $f_i(S)$ (for $i\in\set{1,2,3,4}$) the function that checks whether $S$ satisfied the condition for being an approximate minimal hitting set. Finally, we prove the following proposition.

\begin{proposition}
Let $\signature$ be a schema and let $I$ be an instance of $\signature$. Then, $\forall t_1,t_2 \neg(\overline{P_1}\wedge\dots\wedge \overline{P_n})$ is a $m_i^\epsilon$-approximate DC w.r.t. $I$ if and only if $\set{P_1,\dots,P_n}$ is a $m_i^\epsilon$-minimal hitting set of $Evi_I$.
\end{proposition}
\begin{proof}
Let $S=\set{P_1,\dots,P_n}$ be a set of predicates. Each pair of tuples $\langle t_1,t_2\rangle$ such that $SAT(\langle t_1,t_2\rangle)\cap S\neq\emptyset$ satisfies the DC $\phi=\forall t_1,t_2 \neg(\overline{P_1}\wedge\dots\wedge \overline{P_n})$, since $SAT(\langle t_1,t_2\rangle)$ contains at least one predicate $P_i\in S$ and the pair $\langle t_1,t_2\rangle$ does not satisfy the predicate $\overline{P_i}$ that appears in the DC, thus it does not violate the DC. On the other hand, each pair of tuples $\langle t_1,t_2\rangle$ such that $SAT(\langle t_1,t_2\rangle)\cap S=\emptyset$ violates the DC since $SAT(\langle t_1,t_2\rangle)$ does not contain any predicate from $S$, thus the pair $\langle t_1,t_2\rangle$ satisfies all the predicates in $\overline{S}$ and violates the DC. We now prove the proposition for each one of the definitions.

\paragraph*{$m_1^\epsilon$-approximate DCs} This is straightforward based on the above observation.
\paragraph*{$m_2^\epsilon$-approximate DCs} A set $SAT(\langle t_1,t_2\rangle)$ contains at least $\alpha$ predicates from $\overline{S}$ if and only if the pair $\langle t_1,t_2\rangle$ satisfies at least $\alpha$ of the predicates in the DC $\phi$. This holds since $\phi$ contains exactly the predicates in $\overline{S}$. The rest is implied from this above observation.
\paragraph*{$m_3^\epsilon$-approximate DCs} This is again straightforward based on the above observation.
\paragraph*{$m_4^\epsilon$-approximate DCs} If $S$ is a $m_4^\epsilon$-minimal hitting set of $Evi_I$ then there exists a subinstance $J$ of $I$ such that $|I\setminus J|<\epsilon|I|$ and $S$ is a minimal hitting set of $Evi_J$. Thus, the above observation implies that $\phi$ is a valid DC w.r.t. $J$, and clearly the number of tuples that should be removed for the DC to holds is at most the number of tuples in $I\setminus J$; that is, at most $\epsilon|I|$. For the other direction, if $\phi$ is a $m_4^\epsilon$-approximate DC w.r.t. $I$, then it holds that $|I|-max\set{|J|\mid J\subseteq I, J\models \phi}<\epsilon|I|$ and there exists a subinstance $J$ of $I$ that satisfied $\phi$ such that $|I\setminus J|<\epsilon|I|$. Since $J$ satisfies $\phi$, the above observation implies that $S$ is a minimal hitting set of $Evi_J$.
\end{proof}

\subsection{Properties and Relationships}
We now prove some results regarding the properties of the above definitions and the relationships between them, that we will later use in our mining algorithm. We start by proving that $f_1$, $f_3$ and $f_4$ are anti-monotonic. That is, we prove that $f_i(S)\le f_i(S')$ when $S'\subseteq S$. Since the functions are boolean, this means that if the function returns true for a set $S$, it will also return true for any set that contains $S$.

\begin{proposition}
The functions $f_1$, $f_3$ and $f_4$ are anti-monotonic.
\end{proposition}
\begin{proof}
It is straightforward that $f_1$ is anti-monotonic as the denominator is the number of sets in $Evi_I$ which does not depend on $S$ and adding more predicates to $S$ can only decrease the number of sets in $Evi_I$ that have an empty intersection with $S$. Next, we prove that $f_3$ is anti-monotonic. The denominator is the number of tuples which again does not depend on $S$. Clearly, all the sets that have a nonempty intersection with $S$ also have a nonempty intersection with any set $S'$ such that $S\subseteq S'$. Thus, the number of tuples $t_j\in I$ for which there exists a tuple $t_k\in I$ such that $SAT(\langle t_j,t_k\rangle)\cap S=\emptyset$ or $SAT(\langle t_k,t_j\rangle)\cap S=\emptyset$ can only get smaller when adding more predicates to $S$. Finally, we prove that $f_4$ is anti-monotonic. If $f_4(S)$ is true, there exists a subinstance $J$ of $I$ such that $|I\setminus J|\le \epsilon |I|$ and $S$ has a nonempty intersection with all the sets in $Evi_J$. Clearly, for each set $S'$ such that $S\subseteq S'$ it holds that $S'$ has a nonempty intersection with all the sets in $Evi_J$ as well. Thus, $S'$ also satisfies the condition of $f_4$ with the same subinstance $J$ and $f_4(S')$ is true.
\end{proof}

The function $f_2$ is the only function for which the denominator in the value depends on $S$. The numerator can only get smaller when adding more predicates to $S$, as explained in the above proof for $f_1$, however the denominator can also get smaller. For example, if $S'$ contains all the predicates in $S$ and one more predicate $p$ that appears in all the sets in $Evi_I$, the numerator is the same for both $S$ and $S'$ as none of the sets in $Evi_I$ satisfies $\overline{p}$. However, the denominator for $S'$ can be smaller, as each set in $Evi_I$ satisfies the same amount of predicates in $\overline{S}$ and $\overline{S'}$, but $\overline{S'}$ contains more predicates. In this case, $f(S)$ can be true while $f(S')$ is false, thus the function is not anti-monotonic. Next, we show some relationships between the different definitions.

\begin{proposition}
If $S$ is a $m_2^\epsilon$-minimal hitting set of $Evi_I$ then $S$ is a $m_1^{\epsilon}$-minimal hitting set of $Evi_I$.
\end{proposition}
\begin{proof}
Since $S$ is a $m_2^\epsilon$-minimal hitting set of $Evi_I$, it has an empty intersection with at most $\epsilon$ of the sets in $Evi_I$ that contain at least $\alpha$ of the predicates from $\overline{S}$. In this case, it clearly has an empty intersection with at most $\epsilon$ of the sets in $Evi_I$ as well.
\end{proof}

\begin{proposition}
If $S$ is a $m_3^\epsilon$-minimal hitting set of $Evi_I$ then $S$ is a $m_1^{2\epsilon}$-minimal hitting set of $Evi_I$.
\end{proposition}
\begin{proof}
Each tuple $t$ of $I$ appears in $2(|I|-1)$ sets in $Evi_I$ (as it appears twice with every other tuple). If $S$ is a $m_3^\epsilon$-minimal hitting set of $Evi_I$, then at most $\epsilon|I|$ tuples appear in a violating pair. Thus, the number of violating pairs is at most $2\epsilon|I|(|I|-1)$, which is exactly $2\epsilon$ of the sets in $Evi_I$.
\end{proof}

\begin{proposition}
If $S$ is a $m_4^\epsilon$-minimal hitting set of $Evi_I$ then $S$ is a $m_1^{2\epsilon}$-minimal hitting set of $Evi_I$.
\end{proposition}
\begin{proof}
As mentioned in the previous proof, each tuple $t$ of $I$ appears in $2(|I|-1)$ sets in $Evi_I$. Thus, when we remove a tuple $t$ from $I$, we remove $2(|I|-1)$ sets from $Evi_I$. If $S$ is a $m_4^\epsilon$-minimal hitting set of $Evi_I$, then there is a subinstance $J$ if $I$ such that we removed at most $\epsilon|I|$ tuples from $I$ to obtain $J$ and $S$ is a minimal hitting set of $Evi_J$. The above observation implies that $Evi_J$ contains every set in $Evi_I$ except for at most $2X(|I|-1)$ sets where $X=I\setminus J$. Since $S$ is a minimal hitting set of $Evi_J$, at most $2X(|I|-1)$ sets in $Evi_I$ have an empty intersection with $S$. Thus, we can conclude that the number of sets in $Evi_I$ that have a empty intersection with $S$ is $2X(|I|-1)\le 2\epsilon|I|(|I|-1)$. Hence, at most $2\epsilon$ of the sets in $Evi_I$ have an empty intersection with $S$.
\end{proof}

==> definitions_copy.tex <==
\section{Problem Definition}\label{sec:problem}
%In order to formally define the problem, we first recall some definitions and results given by Chu et al.~\cite{DBLP:journals/pvldb/ChuIP13}. Let $I$ be a database instance. Given a pair $\langle t_1,t_2\rangle$ of tuples from $I$, the \e{satisfied predicates set} for $\langle t_1,t_2\rangle$ is 
%\[SAT(\langle t_1,t_2\rangle)=\set{P\mid P\in\pspace,\set{t_1,t_2}\models P}\]
%That is, $SAT(\langle t_1,t_2\rangle)$ contains all the predicates that are satisfied by $\langle t_1,t_2\rangle$. Then, the \e{evidence set} of $I$ is defined as follows. 
%\[Evi_I=\set{SAT(\langle t_1,t_2\rangle)\mid t_1,t_2\in I}\]
%Note that two distinct pairs of tuples $\langle t_1,t_2\rangle$ and $\langle t_3,t_4\rangle$ may satisfy $SAT(\langle t_1,t_2\rangle)=SAT(\langle t_3,t_4\rangle)$. In our definitions we assume that $Evi_I$ contains a set of predicates for each pair of tuples in $I$, and the number of occurrences of each set is important to us; hence, we treat $Evi_I$ as a \e{bag} rather than a set. Thus, we slightly abuse the notation of a minimal hitting set and use it for bags.
%Chu et al.~\cite{DBLP:journals/pvldb/ChuIP13} proved the following.

%\begin{citedtheorem}{DBLP:journals/pvldb/ChuIP13}\label{thm:reduction-to-hit}
%Let $I$ be a database instance. Then, $\forall t_1,t_2 \neg(\overline{P_1}\wedge\dots\wedge \overline{P_n})$ is a valid minimal DC w.r.t. $I$ if and only if $\set{P_1,\dots,P_n}$ is a minimal hitting set of $Evi_I$.
%\end{citedtheorem}

%{
%\begin{algseries}{t}{\label{alg:fastdc} An algorithm for enumerating minimal valid DCs}
%\begin{insidealg}{FASTDC}{$I,\signature$}
%\STATE $\pspace=\algname{GeneratePredicates}(I,\signature)$ 
%\STATE $Evi_I=\algname{BuildEvidenceSet}(I,P)$ 
%\STATE $MHS=\algname{SearchMinimalCovers}(I,Evi_I,\emptyset,>_{init},\emptyset)$
%\FORALL {$S\in MHS$}
%\STATE $\Sigma = \Sigma \cup \set{\forall t_1,t_2 \neg(\overline{S})}$
%\ENDFOR
%\FORALL {$\phi\in \Sigma$}
%\IF {$(\Sigma\setminus\set{\phi})\models \phi$}
%\STATE $\Sigma = \Sigma\setminus\set{\phi}$
%\ENDIF
%\ENDFOR
%\end{insidealg}
%\end{algseries}
%}

%Recall that the \e{hitting set} problem is the following: given a finite set $K$ and a family $M$ of subsets of $K$, find all the subsets of $K$ that intersect every one of the sets in $M$. A subset $F$ is a \e{minimal} hitting set if no proper subset of $F$ is a hitting set of $M$. Theorem~\ref{thm:reduction-to-hit} holds since by the definition of a hitting set, for each pair of tuples $\langle t_1,t_2\rangle$, the set $SAT(\langle t_1,t_2\rangle)$ contains at least one predicate $P_i\in\set{P_1,\dots,P_n}$; thus, this pair does not satisfy the predicate $\overline{P_i}$ and does satisfy the DC (as a pair of tuples violates a DC if and only if it satisfies all the predicates in it). 

%In order to generate all the valid minimal DCs, Chu et al.~\cite{DBLP:journals/pvldb/ChuIP13} first build the evidence set $Evi_I$ and then generate all the minimal hitting sets for $Evi_I$. In this work we adapt their approach. That is, our problem becomes the problem of finding all the approximate minimal hitting sets for the evidence set $Evi_I$. Thus, we first have to introduce the definition of an approximate hitting set that we consider in this paper. 
In this section, we formally define the problem that we study in the paper.
We start by defining a \e{valid approximation function}.
Let $D$ be a database and let $S$ be a set of predicates. Let $f$ be a function $f:(D,S)\rightarrow [0,1]$. We now define the following two properties of such a function $f$.

\begin{definition}[Monotonicity]
A function $f:(D,S)\rightarrow [0,1]$ is monotonic if $f(D,S)\le f(D,S')$ whenever $S\subset S'$.
\end{definition}

Intuitively, it is harder to violate a DC that contains more predicates, as more conditions have to hold. Monotonicity ensures that the more predicates $S$ contains, the higher its score is (as the number of pairs of tuples satisfying all the predicates in $S$ can only increase).
As mentioned in the introduction, monotonicity allows us to consider only minimal ADCs (i.e., ADCs that do not strictly contain any ADC), as it assures that whenever $\phi$ is an ADC, every $\phi'$ such that $S_\phi\subset S_{\phi'}$ is also an ADC. Hence, when we return only minimal ADCs $\phi$, we also implicitly provide the user with information on any $\phi'$ that can be obtained from $\phi$ by adding more predicates. For non-monotonic functions, on the other hand, it may be the case, for example, that for $\phi,\phi'$ and $\phi''$ such that $S_\phi\subset S_{\phi'}\subset S_{\phi''}$, while $\phi$ and $\phi''$ are ADCs, $\phi'$ is not. In this case, returning only $\phi$ will result is the loss of valuable information, and it will be necessary to go over the entire space of possible ADCs to make sure that we return all of them. We now move on to the second property.

\begin{definition}[Indifference to Redundancy]
A function $f:(D,S)\rightarrow [0,1]$ is indifferent to redundancy if whenever $S\subset S'$ and $\set{F\mid F\in \evi(D), S\cap F\neq\emptyset}=\set{F\mid F\in \evi(D), S'\cap F\neq\emptyset}$, we have that $f(D,S)=f(D,S')$.
\end{definition}

Intuitively, a function $f$ is indifferent to redundancy if adding more elements to a set $S$ without affecting the coverage, does not affect the score. That is, if two sets $S\subset S'$ have a nonempty intersection with the exact same sets in $\evi(D)$, then we assume that $f$ gives them the same score. While our algorithm for enumerating minimal approximate hitting sets could work for functions that do not satisfy indifference to redundancy, having this property allows us to significantly increase the efficiency of our algorithm by pruning branches in the search tree early, as we will explain in Section~\ref{sec:algorithm}. 
We now introduce the definition of a valid approximation function in our setting.

\begin{definition}[Valid Approximation Function]
A function $f:(D,S)\rightarrow [0,1]$ is a valid approximation function if it satisfies monotonicity and indifference to redundancy.
\end{definition}

The intuition behind combining both properties is illustrated in the following example.

\begin{example}
consider the following DCs:
\[\phi=\forall t_1,t_2 \neg(t_1.A<t_2.A\wedge t_1.A\le t_2.A)\]
\[\phi'=\forall t_1,t_2 \neg(t_1.A<t_2.A)\]
Clearly, the set $S_{\phi'}$ has a nonempty intersection with the exact same sets from $\evi(D)$ as $S_\phi$, since whenever a tuple pair satisfies the predicate $t_1.A<t_2.A$ it also satisfies $t_1.A\le t_2.A$. Intuitively, the DC $\phi'$ is minimal, while $\phi$ is not minimal, as there is no benefit in adding the predicate $t_1.A\le t_2.A$ to the DC (it does not make the DC ``more correct''). For a monotonic function $f$, it will hold that $f(D,S_{\phi'})<f(D,S_\phi)$; however, it may be the case that $1-f(D,S_\phi)<\epsilon$, while $1-f(D,S_{\phi'})>\epsilon$, in which case we will return $\phi$ and not $\phi'$. The existence of the second property that we introduced (indifference to redundancy) resolves this problem, as $\set{F\mid F\in \evi(D), S_\phi\cap F\neq\emptyset}=\set{F\mid F\in \evi(D), S_{\phi'}\cap F\neq\emptyset}$; thus, we have that $f(D,S_\phi)=f(D,S_{\phi'})$ and we will either return $\phi'$ (if $1-f(D,S_{\phi'})<\epsilon$) or we will not return any of these DCs.
\end{example}

In the next section, we will show that our definition of a valid approximation function is quite general, as it captures common approximation functions. Next, we give the formal definition of an approximate minimal hitting set.

\begin{definition}[Minimal Approximate Hitting Set]
Let $K$ be a finite set of elements, and let $M$ be a set of subsetss of $K$. In addition, let $f$ be a valid approximation function and let $\epsilon>0$. Then, $S\subset K$ is a minimal approximate hitting set of $M$ w.r.t~$f$ if it satisfies the following:
\begin{enumerate}
\item It holds that $1-f(D,S)<\epsilon$,
\item There is no set $S'\subset K$ such that $S'\subset S$ and $1-f(D,S')<\epsilon$.
\end{enumerate}
\end{definition}

Note that when using the following approximation function:
\[
f(D,S) \eqdef
\begin{cases}
1 & \mbox{$S\cap F\neq\emptyset$ for all $F\in \evi(D)$} \\ 
0 & \mbox{otherwise}\\ 
\end{cases}
\]
we obtain exactly the definition of a minimal hitting set. This function satisfies both monotonicity and indifference to redundancy; hence, our algorithm can be used for enumerating valid DCs as well. Moreover, existing algorithms for enumerating minimal hitting sets use these properties to effectively prune the search space. By assuming that a valid approximation function satisfies both properties, we are able to use these pruning techniques to prune the search space in our problem as well.

Finally, we define a minimal approximate DC.

\begin{definition}[Minimal Approximate Denial Constraint]
Let $D$ be a database, let $f:(D,S)\rightarrow [0,1]$ be a valid approximation function, and let $\epsilon>0$. Then, a DC $\phi$ is a minimal approximate DC if $S_{\phi}$ is a minimal approximate hitting sets of $\evi(D)$ w.r.t.~$f$.
\end{definition}

Finally, we define the problem that we study in this paper. Let $I$ be a database instance and let $\epsilon>0$. The \e{mining problem} for approximate DCs is to find all the nontrivial $\epsilon$-approximate DCs for $I$. In Section~\ref{sec:algorithm} we introduce a mining algorithm that solves the mining problem for any valid approximation function (we introduce different valid approximation functions in the next section). In Section~\ref{sec:sample} we explain how we can solve the problem using only a sample of the data, while getting good DCs.

%To generate all the minimal hitting sets, they use their own algorithm. In order to generate the approximate DCs, they modify this algorithm to generate approximate hitting sets instead. Since Chu et al.~\cite{DBLP:journals/pvldb/ChuIP13} only considered $m_1^\epsilon$-approximate DCs (that is, DCs that are violated by at most $\epsilon$ of the tuple pairs for some $\epsilon>0$), they defined an approximate hitting set ($\epsilon$-minimal hitting set) as a set that has an empty intersection with at most $\epsilon$ of the subsets. This definition is also used in other works that consider approximate hitting sets in other domains~\cite{VINTERBO2000123, Rioult2010}. We refer to this definition of approximate hitting sets as $m_1^\epsilon$-minimal hitting set to avoid confusion. We now give the formal definition.
%
%
%
%
%
%
%
%
%To the best of our knowledge, the only work that has considered approximate DCs so far is that of Chu et al.~\cite{DBLP:journals/pvldb/ChuIP13}. They defined an approximate DC as a DC that is satisfied by most of the pairs of tuples in the database instance. However, this is not the only possible definition that can be used. Kivinen et al.~\cite{Kivinen1992} introduced three definitions for approximate FDs, based on three different measures for the number of violations of the FD in the database. These three definitions can be easily extended for DCs. We start by discussing each one of these measures.
%
%Let $I$ be a database instance and let $\psi=X\rightarrow Y$ be an FD. The first definition is based on the following measure. 
%\[G_1(\psi)=\left|\set{\langle t_1,t_2 \rangle\mid t_1,t_2\in I, t_1[X]=t_2[X], t_1[Y]\neq t_2[Y]}\right|\]
%\[g_1(\psi)=G_1/|I|^2\]
%That is, $g_1$ is the number of pairs of tuples that violate the FD (agree on the value of all the attributes in $X$, but do not agree on the value of at least one attribute in $Y$), divided by the total number of pairs of tuples. Intuitively, this is the probability to select a violating pair of tuples among all pairs, assuming a uniform distribution. For a DC $\phi$, we can use this measure as follows:
%\[m_1(\phi)=\left|\set{\langle t_1,t_2 \rangle\mid t_1,t_2\in I, \set{t_1,t_2}\not\models\phi}\right|/\left[|I|\cdot(|I|-1)\right]\]
%Note that in the original definition the denominator is $|I|^2$, while in our definition the denominator is $|I|\cdot(|I|-1)$, as a tuple will never violate a constraint with itself, thus we do not need to count the number of pairs $\langle t_1,t_2 \rangle$ where $t_1=t_2$. In fact, using $|I|\cdot(|I|-1)$ as the denominator has its disadvantages as well. In the case of $g_1$ (the measure for FDs), note that a pair of tuples $\langle t_1,t_2 \rangle$ that satisfies $t_1[X]\neq t_2[X]$ affects the measure, even though this pair of tuples does not really provide us with any information about the relationship between $X$ and $Y$. A similar argument can be made for DCs. If a pair of tuples does not agree on any of the predicates in a DC $\phi$, it is not clear if this pair should affect the measure $m_1$, or if it should affect the measure in the same way as a pair that satisfies most of the predicates affects it.
%
%To resolve this problem, we propose a slightly different measure that takes into account the number of predicates from the DC that are satisfied by a pair of tuples. Here, we do not consider all the pairs in the denominator, but only those that satisfy at least $\alpha$ of the predicates in the DC, for some $0<\alpha<1$. Note that we do not fix a specific value of $\alpha$, but we will later experimentally compare different values. This measure is somehow related to the \e{coverage} measure proposed by Chu et al.~\cite{DBLP:journals/pvldb/ChuIP13} for ranking DCs, as we discuss in Section~\ref{sec:ranking}. The idea there is the following: the more predicates from the DC a pair satisfies, the higher the affect this pair has on the rank score. Following Chu et al.~\cite{DBLP:journals/pvldb/ChuIP13}, we denote by \e{kE} (k-evidence) the set of tuple pairs that satisfy $k$ predicates from a DC $\phi$. Formally, we propose the following measure.
%\[d=\sum_{k=\lceil\alpha\cdot|\varpi(\phi)|\rceil}^{|\varpi(\phi)|} \left|\set{\langle t_1,t_2 \rangle\mid t_1,t_2\in I, \langle t_1,t_2 \rangle\in kE}\right|\]
%\[m_2(\phi)=\left|\set{\langle t_1,t_2 \rangle\mid t_1,t_2\in I, \set{t_1,t_2}\not\models\phi}\right|/d\]
%
%
%
%%The idea is the following: the more predicates from the DC the pair satisfies, the higher the affect this pair has on the measure. This measure is closely related to the \e{coverage} measure proposed by Chu et al.~\cite{DBLP:journals/pvldb/ChuIP13} for ranking DCs, as we discuss in Section~\ref{sec:ranking}. We change the denominator in the following way. If a pair $\langle t_1,t_2 \rangle$ satisfies $k$ out of $m$ predicates from the DC, for some $0\le k\le m-1$, then we add the value $(k+1)/m$ to the denominator. Since we are studying approximte DCs, there may also be pairs of tuples that satisfy all the predicates in the DC. As we consider pairs of tuples that satisfy all the predicates in the DC except one and pairs of tuples that satisfy all the predicates in the DC equally informative (as the first type indicates that the DC is correct and the second one indicates that it is incorrect), we give the same weight $1$ for these pairs. Following Chu et al.~\cite{DBLP:journals/pvldb/ChuIP13}, we denote by \e{kE} (k-evidence) the set of tuple pairs that satisfy $k$ predicates from a DC $\phi$. Formally, we propose the following measure.
%%\[w_k=min\set{(k+1)/|\varpi(\phi)|,1}\]
%%\[d=\sum_{k=0}^{|\varpi(\phi)|} \left|\langle t_1,t_2 \rangle\mid t_1,t_2\in I, \langle t_1,t_2 \rangle\in kE\right|\cdot w_k\]
%%\[m_2(\phi)=\left|\langle t_1,t_2 \rangle\mid t_1,t_2\in I, \set{t_1,t_2}\not\models\phi\right|/d\]
%
%The second definition of Kivinen et al.~\cite{Kivinen1992} is based on the following measure.
%\[G_2(\psi)=\left|\set{t_1\mid t_1\in I, \exists t_2\in I, t_1[X]=t_2[X], t_1[Y]\neq t_2[Y]}\right|\]
%\[g_2(\psi)=G_2/|I|\]
%That is, $g_2$ is the number of tuples that violate the FD with at least one other tuple (or in other words, the number of tuples that participate in a violation of the FD), divided by the total number of tuples. Intuitively, this is the probability to select a violating tuple among all tuples, assuming a uniform distribution. We can again easily generalize this measure to DCs, using the following definition.
%\[m_3(\phi)=\left|\set{t_1\mid t_1\in I, \exists t_2\in I, \set{t_1,t_2}\not\models \phi}\right|/|I|\]
%
%In the case of inconsistent database instances, for example, it may be the case that there is only one dirty tuple, but all the pairs of tuples that include this tuple violate the DC. In this case, it holds that $g_2=1$, as all the tuples appear in one violating pair. However, if we just remove this one tuple, the DC will hold. Thus, this measure may be too sensitive in the case of dirty data, and the last measure proposed by Kivinen et al.~\cite{Kivinen1992} seems to be a better fit in this case. Their last definition is based on the following measure.
%\[G_3(\psi)=n-max\set{|J|\mid J\subseteq I, J\models (X\rightarrow Y)}\]
%\[g_3(\psi)=G_3/|I|\]
%That is, $g_3$ is the minimum number of tuples that should be removed from $I$ for the FD to hold. The subinstance $J$ of $I$ that is considered in this measure is the \e{cardinality repair}~\cite{DBLP:conf/icdt/LopatenkoB07} of $I$ (that is, the largest subinstance of $I$ among all those satisfying the FD). $J$ can also be seen as a Most Probable Database~\cite{Gribkoff2014TheMP}: given the FD $X\rightarrow Y$, the subinstance $J$ is the subinstance that has the highest probability among all the subinstances of $I$ that satisfy the FD, assuming that all tuples have the same probability $p\ge 0.5$. The following version of the measure can be used for DCs.
%\[m_4(\phi)=\left(n-max\set{|J|\mid J\subseteq I, J\models \phi}\right)/|I|\]
%
%Next, we give the formal definition of an approximate DC that we consider in this paper.
%
%\begin{definition}[Approximate DC]
%Let $\signature$ be a schema and let $I$ be an instance of $\signature$. Let $\epsilon>0$. An $m_i^\epsilon$-approximate DC is a nontrivial minimal DC $\phi$, such that $m_i(\phi)<\epsilon$.
%\end{definition}
%
%We say that an approximate DC $\phi$ is \e{minimal} if no other DC $\phi'$ such that $\varpi(\phi')\subset\varpi(\phi)$ satisfies $m_i(\phi')<\epsilon$. Finally, we define the problem that we are studying in this paper. Let $\signature$ be a schema and let $I$ be an instance of $\signature$. Let $\epsilon>0$. The \e{mining problem} for approximate DCs is to find all the $m_i^\epsilon$-approximate DCs for $i\in\set{1,2,3,4}$.
%
%\subsection{Complexity}
%Unlike the first three measures ($m_1$, $m_2$ and $m_3$), which can be computed in polynomial time for both FDs and DCs, the fourth measure ($m_4$) can be computed in polynomial time for FDs~\cite{DBLP:journals/corr/abs-1712-07705}, but for DCs this is a hard problem~\cite{DBLP:conf/icdt/LopatenkoB07}. Lopatenko et al.~\cite{DBLP:conf/icdt/LopatenkoB07} have shown that finding the minimum number of tuples to remove from a database for a DC to hold is complete for $FP^{NP(log(n))}$ for a DC that involves three relations. We now prove that the problem is hard even in our more restricted version of DCs, where we only consider a single relation schemas.
%
%\begin{theorem}\label{thm:m4-hard}
%Let $I$ be a database instance. Then, finding the minimum number of tuples that should be removed from $I$ for a DC to holds is NP-hard.
%\end{theorem}
%\begin{proof}
%We construct a reduction from the problem of finding the maximum independent set of a graph. The input to this problem is a graph $g$.
%The goal is to find a maximum size set $S$ of vertices such that for every two vertices $v_1,v_2$ in $S$, there is no edge $(v_1,v_2)$ in $g$. This problem is known to be NP-hard.
%Given such an input, 
% we will construct the input 
% $I$ over the relation $R(A_1,\dots,A_{|V(g)|^2})$ for our problem as follows.
% Let $\set{v_1,\dots,v_n}$ be the set of vertices in $g$. For each vertex $v_i$ in $g$, the instance $I$ will contain a tuple $t_i=(a^i_{1,1},\dots,a^i_{n,n})$, where:
%\[
%a^i_{k,l} =
%\begin{cases}
%i & \mbox{$k\neq i$ and $l\neq i$} \\ 
%\langle k,l\rangle & \mbox{$k=i$ and $(v_k,v_l)\in E(g)$} \\ 
%\langle l,k\rangle & \mbox{$l=i$ and $(v_k,v_l)\in E(g)$} \\ 
% \langle min(k,l),max(k,l)\rangle& \mbox{otherwise}
%\end{cases}
%\]
%
%The DC  $\phi$ will be $\forall t_1,t_2\neg(t_1.{A_1}\neq t_2.{A_1},\dots, t_1.A_{n^2}\neq t_2.A_{n^2})$. We will now prove that each subinstance $J$ of $I$ for which the DC holds corresponds to an independent set of $g$ and vice versa.
% 
%\paragraph*{Subinstance to independent set}
%Let $J$ be a subinstance of $I$, such that $\phi$ is a valid DC for $J$. We claim that the set $S=\set{v_{j_1},\dots,v_{j_m}}$ that contain a vertex $v_{j_r}$ for each tuple $t_{j_r}$ in $J$ (and only these vertices) is an independent set. Let us assume, by way of contradiction, that there are two vertices $v_{j_r}$ and $v_{j_p}$ in $S$ such that $(v_{j_r},v_{j_p})\in E(g)$. The tuples $t_{j_r}$ and $t_{j_p}$ clearly disagree on each value $a_{k,l}$ where at least one of them is missing (that is, either $k\neq j_r$ and $l\neq j_r$ or $k\neq j_p$ and $l\neq j_p$). In addition, it holds that $a^{j_r}_{j_r,j_p}=a^{j_r}_{j_p,j_r}=\langle j_r,j_p\rangle$ while $a^{j_p}_{j_r,j_p}=a^{j_p}_{j_p,j_r}=\langle j_p,j_r\rangle$. Thus, $t_{j_r}$ and $t_{j_p}$ disagree on the value of all the attributes and violate the DC, which is a contradiction to the fact that $J$ satisfies $\phi$.
%
%\paragraph*{Independent set to subinstance}
%Let $S=\set{v_{j_1},\dots,v_{j_m}}$ be an independent set of $g$. We claim that the subinstance $J$ of $I$ that contains each tuple $t_j$ for $j\in\set{i_1,\dots i_m}$ (and only these tuples) satisfies $\phi$. If two tuples $t_{i_r},t_{i_p}$ in $J$ violate $\phi$ then they agree on all the predicates in $\phi$. This means that they disagree on the value of all the attributes. However, it holds that $a_{i_r,i_p}=\langle min(i_r,i_p),max(i_r,i_p)\rangle$ for both tuples (as $S$ is an independent set, thus there is no edge between the corresponding vertices). That is, the two tuples agree on the attribute that contains the value $a_{i_r,i_p}$, and they cannot violate the DC.
%\end{proof}
%
%Theorem~\ref{thm:m4-hard} implies that we cannot efficiently calculate the $m_4$ measure. However, there is a simple reduction from the problem of finding the minimum number of tuples to remove for a DC to hold to the minimum vertex cover problem. The reduction is based on the concept of a \e{conflict graph}~\cite{10.1007/3-540-44503-X_3} which is a graph that has a vertex for each tuple in the database and an edge between two tuples that violate the DC. It is straightforward that the size of the minimum vertex cover of the conflict graph is exactly the minimum number of tuples to remove (as we have to remove at least one tuple for each pair of conflicting tuples). As vertex cover is 2-approximable in polynomial
%time~\cite{DBLP:journals/jal/Bar-YehudaE81}, we can conclude that this is also the case for our problem.
%
%%\begin{comment}
%%Although in this paper we only consider four possible definitions of approximate DCs, the algorithm that we provide in the next section actually works for \e{any} definition of approximate DCs, as long as the \e{minimality} definition is not modified. Thus, from now on, we refer to general approximate DCs (that is, when the definition does not matter) as approximate DCs, and to our specific definitions of approximate DCs as $m_i$-approximate DCs.
%%\end{comment}
%


==> multiple.tex <==
\section{Multiple DCs}

==> proof.tex <==
\begin{proof}
\ester{The proofs of \e{(a)} and \e{(c)} are rather straightforward, and we give them in the extended version of the paper~\cite{}. Here, we focus on \e{(b)}.}
% The first part is straightforward, as we return a set $S$ only if $1-f(D,S)\le \epsilon$ and $S$ is minimal. For the last part, observe that the two recursive calls in each iteration cannot result in the same $S$ (since in the first one $S$ will always have an empty intersection with the selected $F$, while in the second one $S$ will have a nonempty intersection with $F$). Moreover, the first recursive call does not modify $S$, while the second one is identical to the recursive call of the algorithm $\algname{MMSC}$. We conclude that since $\algname{MMSC}$ returns every minimal hitting set once, our algorithm returns every minimal approximate hitting set once.
We prove by induction on $n$, the depth of the recursion, that $\algname{ADCEnum}(S,\crit,\uncov,\cand,\canCover)$ returns every minimal ADC $\varphi$ that satisfies:
\begin{citemize}
\item $S\subseteq S_\varphi$ and $S_\varphi\subseteq (S\cup \cand)$,
\item $S_\varphi$ has an empty intersection with all the sets $F\in \evi(D)$ for which $\canCover[F]=\mbox{false}$.
\end{citemize}
Note that the sets for which $\canCover[F]=\mbox{true}$ can either have an empty or a nonempty intersection with $S_\varphi$. Since at the beginning, $\cand$ contains all the predicates of $\pspace_R$ and we have that $\canCover[F]= \mbox{true}$ for each $F\in \evi(D)$, we will conclude that $\algname{ADCEnum}(\emptyset,\crit,\uncov,\cand,\canCover)$ returns every ADC $\varphi$ such that $\emptyset\subseteq S_\varphi$ and $S_\varphi\subseteq \cand$; that is, all the ADCs.

For the basis of the induction, $n=0$, one possible case is that the condition of line~1 holds. Then, the constraint corresponding to $S$ itself is a minimal ADC; thus, the only $S_\varphi$ that contains $S$ such that $\varphi$ is a minimal ADC is $S$ itself, and we indeed return $S$. Note that the sets $F$ for which it holds that $\canCover[F]=\mbox{false}$ have an empty intersection with $S$, as we update the value $\canCover[F]$ for a set $F$ to false only when $\cand$ no longer contains any predicate of $F$. If the condition of line~1 does not hold, then the only other option is that the condition of line~5 holds. In this case, no $S_\varphi$ that contains $S$ is such that $\varphi$ is an ADC, as it does not holds that $1-f(D,S)\le\epsilon$ and the remaining candidate predicates do not appear in any of the remaining sets in $\uncov$.

For the inductive step, we prove that if the claim holds for all $n\in\set{1,\dots,k-1}$, it also holds for $n = k$. Let us consider an iteration from which the depth of the recursion is $k$. In line~4, we choose a set $F$ for which $\canCover[F]=\mbox{true}$. Each $S_\varphi$ that contains $S$ either has a nonempty intersection with $F$ or an empty one. In the first case, let $S_\varphi$ be a minimal ADC that has a nonempty intersection with $F$ and satisfies the two conditions. In line~14, we go over all the predicates of $F$ and try to add each one of them to $S$.  Clearly, $S_\varphi$ contains at least one of these predicates. Let $\set{p_1,\dots,p_k}=S_\varphi\cap F$ and assume that $p_1,\dots,p_k$ is the order by which they are selected in line~14. We claim that $S_\varphi$ is generated in the recursive call made when $p_k$ is selected in line~14.

Each predicate of $\set{p_1,\dots,p_k}$ is in $\cand$ at this point, since we assume that $S_\varphi\subseteq (S\cup\cand)$ and none of these predicates can violate the minimality condition of line~17, as this will imply that $S_\varphi$ contains an element that is not critical for any subset, which is a contradiction to the fact that $S_\varphi$ is minimal (due to indifference to redundancy). Hence, every predicate in $\set{p_1,\dots,p_k}$ is added back to $\cand$ in line~20, and since $p_k$ is the last predicate selected in the loop of line~15, in that iteration all the other predicates already belong to $\cand$. From the inductive assumption, we know that $\algname{ADCEnum}$ generates every minimal ADC that contains $S\cup \set{p_k}$, is contained in $S\cup \set{p_k}\cup \cand$, and has an empty intersection with every $F'$ for which $\canCover[F']=\mbox{false}$, when given the set $S\cup \set{p_k}$ as input; among them is $S_\varphi$ (observe that we do not change the data structure $\canCover$ for the recursive call of line~19).

For the second case, let $S_\varphi$ be a minimal ADC that has an empty intersection with $F$ and satisfies the two conditions. We claim that $S_\varphi$ is generated in the recursive call of line~10. Here, we make a recursive call with the same $S$ after removing all the predicates of $F$ from $\cand$, and updating $\canCover[F']$ to false for each $F'$ that no longer contains any predicates from $\cand$. From the inductive assumption, we know that this recursive call generates every minimal ADC that contains $S$ and has an empty intersection with $F$ (as no predicate of $F$ appears in $\cand$); among them is $S_\varphi$. That concludes our proof of correctness for the algorithm.
\end{proof}

==> ranking.tex <==
\section{Ranking DCs}

As the number of approximate DCs can be very large, we would like to have a ranking method that will enable us to return only the $k$ most meaningful DCs. In this section we discuss some ranking methods. We start by discussing the \e{interestingness} score proposed by Chu et al.~\cite{} for ranking DCs.
This score is a linear weighted combination between two measures. The first one measures the length of the DC such that the shorter the DC, the higher this measure is. Formally, the \e{succinctness} of a DC $\phi$ is defined as follows.
\[Succ(\phi)=\frac{Min\{Length(\phi')\}}{Length(\phi)}\]
That is, $Succ(\phi)$ is the length of the minimum DC divided by the length of $\phi$. Clearly, it holds that $0\le Succ(\phi)\le 1$. To measure the length of the DC, Chu et al.~\cite{} propose to count the number of symbols from $\set{t_1,t_2,A,O,Cons}$ that appear in the DC, where $A$ is the set of attributes, $O$ is the set of operators and $Cons$ are constants. 

The second measure, \e{coverage}, is closely related to our definition of $m_2$-approximate DCs and is defined as follows.
\[Coverage(\phi)=\frac{\sum_{k=0}^{|\phi.Pres|} |kE|\cdot w_k}{|Evi_I|}\]
We recall that $kE$ contains all the tuple pairs that satisfy $k$ predicates from the DC. Moreover, the weight $w_k$ is defined as $(k+1)/|\phi.Pres|$ for $0\le k \le |\phi.Pres|-1$. That is, each pair of tuples that satisfies $k$ predicates from $\phi$ for $0\le k \le |\phi.Pres|-1$ contributes $w_k$ to the numerator. The denominator is the total number of tuple pairs. Since Chu et al.~\cite{} considered in their work DCs that are satisfied by all tuple pairs, $kE$ is empty for $k=|\phi.Pres|$, thus they did not need to define $w_{|\phi.Pres|}$. As in this work we are considering approximate DC, there may also be pairs of tuples that satisfy all the predicates in the DC (that is, violate the DC). Thus, we also need to consider these pairs in the coverage measure. As we did in the $m_2$ measure, we define $w_{|\phi.Pres|}=1$.

As noted by Chu et al.~\cite{}, $w_k$ can also be 

==> sampling_backup.tex <==
\newcommand{\Prob}{\mathrm{Pr}}

% !TEX root=main.tex
\section{Mining ADCs From a Sample}\label{sec:sample}
 The input to our algorithm is the evidence set
and the complexity of building it is quadratic in the size of
the database (as we have to go over all pairs of tuples), which can be
prohibitively expensive for large databases. In this section, we show
how to use a sample from the database to produce ADCs with 
probabilistic guarantees, while avoiding the cost of building the
evidence set for the entire database~\cite{heidari2019approximate}.
For simplicity, we limit our discussion to a simple approximation
function, namely, the function $f_1$ introduced in 
Section~\ref{sec:functions}. Recall that the function $f_1$ is based
on the number of violations of the DC in the database. 
%that is,
%\[f_1(D,S_\phi)=\left|\set{\langle t,t' \rangle\mid t,t'\in D, \{t,t'\}\models\phi}\right|/|D|^2\]

Let $J$ be a sample uniformly drawn from the input database $D$ and let $\epsilon\ge 0$. Let $\phi$ be an ADC. We address the following two problems: \e{(1)} how to estimate the number of violations of $\phi$ in $D$ from $J$; and \e{(2)} how to use this estimate to decide on the right $\epsilon'$ to be used when enumerating the ADCs from $J$.

%(3) we discuss the minimum sample size needed to produce $ \epsilon -approximate $ DC from sample with guarantees (Section \ref{sec:min}).


\subsection{Estimating the Number of Violations}
\label{sec:vionum}
Since we consider the approximation function $f_1$ that is based on
the number of violations of the DC in the database, we now show how to
estimate this number from a sample $J$ uniformly drawn from $D$. 
We represent the violations of an ADC $\phi$ as a  conflict graph~\cite{DBLP:journals/iandc/ChomickiM05}
$G(V,E)$, where $V$ is the set of vertices corresponding to the tuples
in $D$, and $E$ is the set of edges corresponding to violations of the
DC, where an edge $(t_1,t_2)$ exists if the pair $(t_1,t_2)$ violates the DC. Note that this is a directed graph since a pair $(t_1,t_2)$ may violate a DC that is satisfied by $(t_2,t_1)$.

Let $p=\frac{|E|}{2\cdot {|V|\choose 2}}$ (that is, $p=1-f_1(D,S_\phi)$). Let $G_J(V_J,E_J)$ be the conflict graph of $J$.
To estimate $p$ from $J$, we use $\hat{p}$ defined as follows: $\hat{p}=\frac{|E_J|}{2\cdot {|V_J|\choose 2}}$.  We define the random variable $x_i$ for each pair of nodes in $V_J$, where $x_i = 1$ with probability $p$ and $x_i=0$ with probability $1-p$.
%Observe that while we assume that the probability of an edge in the conflict graph is $p$, 
It can easily shown that $E(\hat{p}) = p$, so it is an unbiased estimator of $p$. 
Note that we do not make assumptions about the structure of the conflict graph or about the dependencies between the edges. 

%We now show that $\hat{p}$ is an unbiased estimator of $p$.
% Now, we can compute $E(\hat{p})$:
% \begin{align*}
% &E(\hat{p})=E\left(\frac{|E_J|}{{|V_J|\choose 2}}\right)=
% E\left(\frac{\sum\limits_{i=1}^{|V_J|\choose 2}x_i}{{|V_J|\choose 2}}\right)=\frac{1}{{|V_J|\choose 2}}E\left(\sum\limits_{i=1}^{|V_J|\choose 2}x_i\right)=\\
% &= \frac{1}{{|V_J|\choose 2}} \sum\limits_{i=1}^{|V_J|\choose 2}E(x_i)=\frac{1}{{|V_J|\choose 2}}\sum\limits_{i=1}^{|V_J|\choose 2}p=
% \frac{1}{{|V_J|\choose 2}}{|V_J|\choose 2}p=p
% \end{align*}

 We further derive error bounds on our estimator to help us derive our guarantees. To compute error bounds, various methods can be used such as Chebyshev's inequality and normal distribution assumption. Most of them require estimating the variance of our estimator.
Here, we use Chebyshev's inequality:
\begin{equation*}
\Prob(|\hat{p}-E(\hat{p})|>a)\leq \frac{1}{a^2}\cdot\var(\hat{p})
\end{equation*}

We know that $p=E(\hat{p})$; hence, we now compute an upper bound on $\var(\hat{p})$. 

\begin{align*}
\var(\hat{p})&=\var\left(\frac{|E_J|}{2\cdot {|V_J|\choose 2}}\right)=\frac{1}{4\cdot {|V_J|\choose 2}^2}\left[E(E_J^2)-E(E_J)^2\right]\\
&=\frac{1}{4\cdot {|V_J|\choose 2}^2}\left[E(E_J^2)-4\cdot {|V_J|\choose 2}^2\cdot p^2\right]
\end{align*} 

We now expand the term $E(E_J^2)$ using the random variables $x_1,\dots,x_{2{|V_J|\choose 2}}$ as follows. 
\begin{align*}
E(E_J^2)&=E\left(\left(\sum\limits_{i=1}^{2\cdot{|V_J|\choose 2}}x_i\right)^2\right)=\\
&=\sum\limits_{i=1}^{2\cdot{|V_J|\choose 2}}E(x_i^2)+\sum\limits_{i\neq j\in \{1,\dots,2\cdot {|V_J|\choose 2}\}} E(x_i\cdot x_j)
\end{align*}

Since we do not assume anything about the dependencies between the variables $x_i$, we cannot calculate the exact value of $E(x_i\cdot x_j)$; however, we can derive an upper bound for this value. We know that $x_i\cdot x_j=1$ if and only if $x_i=x_j=1$, and the value of $E(x_i\cdot x_j)$ depends of the number of these events. Hence, if we can find an upper bound for the probability of $x_i\cdot x_j=1$, this will be an upper bound for $E(x_i\cdot x_j)$. We have the following.
\begin{align*}
& E(x_i\cdot x_j)=\Prob(x_i=1,x_j=1)=\\
&=\Prob(x_i=1|x_j=1)\cdot \Prob(x_j=1)\leq
 \Prob(x_j=1)=p
\end{align*}

Clearly, for $i=j$ it holds that $\Prob(x_i=1,x_j=1)=p$. Hence, we obtain the following upper bound on $E(E_J^2)$.
\begin{align*}
& E(E_J^2)=\sum\limits_{i=1}^{2\cdot {|V_J|\choose 2}}E(x_i^2)+\sum\limits_{i\neq j\in \{1,\dots,2\cdot {|V_J|\choose 2}\}} E(x_i\cdot x_j)=\\
&\leq 2\cdot {|V_J|\choose 2}\cdot p + {2\cdot {|V_J|\choose 2}\choose 2}\cdot p
\end{align*}

Next, we use the upper bound on $E(E_J^2)$ to obtain an upper bound for $\var(\hat{p})$.
\begin{align*}
\var(\hat{p})\leq p\cdot\left[\frac{2\cdot {|V_J|\choose 2}+{2\cdot {|V_J|\choose 2}\choose 2}}{4\cdot{|V_J|\choose 2}^2}-p\right]
\end{align*} 

Using Chebyshev's inequality we obtain the following:

\begin{align*}
\Prob(|\hat{p}-p|>a)\leq \frac{p}{a^2}\cdot\left[\frac{2\cdot {|V_J|\choose 2}+{2\cdot {|V_J|\choose 2}\choose 2}}{4\cdot {|V_J|\choose 2}^2}-p\right]
\end{align*}

The obtained bounds are loose since we did not assume anything about the structure of the conflict graph and the dependencies among the violations. 
%Since Chebyshev's inequality is generally true, it provides weak error bounds in general and adding assumptions on the dependencies among the violations is required to obtain better bounds. 
We now show that better bounds can indeed be obtained under the assumption that violations (or, equivalently, edges) are introduced randomly and independently.

We first introduce the rationale behind random violations as follows. Assume a random polluter which is a probability distribution over graphs on $n$ labeled vertices, where each directed edge appears independently with probability $p$. Each violation (edge) independently occurs between two tuple without following any specific pattern. This assumption helps us find a distribution for $\hat{p}$.
Since the edges are independent, we can calculate $\var(|E_J|)$ (and also $\var(\hat{p})$) accurately. Moreover, the number of edges in a sample $J$ produces a binomial distribution. 
\begin{align*}
\Prob[E_J=i]={2\cdot {|V_J| \choose 2} \choose i}\cdot p^i\cdot (1-p)^{2\cdot {|V_J|\choose 2}-i}
\end{align*}

%There are many approximation methods that can be used such as the normal approximation, the Wilson score interval, the Jeffreys interval, and the Clopper-Pearson interval to approximate $p$ using the estimator $\hat{p}$. 

For simplicity, we assume that the sample size is not too small and $p$ is not too close to $0$ or $1$; 
%so we can use the normal approximation of the binomial distribution; 
hence, we can approximate the binomial $B(n,p)$ under the mentioned conditions using the normal distribution $N(np,np(1-p))$, and we can define a confidence interval parameterized by a confidence level $1-2\alpha$, and $n=2\cdot{|S|\choose 2}$. The confidence interval of normal distribution is given by the following equation.

\begin{equation}
\label{eq:dist}
\Prob\bigg[|p-\hat{p}|\leq z_{1-2\alpha}\cdot\sqrt{\frac{\hat{p}(1-\hat{p})}{n}}\bigg]\geq 1-2\alpha
\end{equation}

In the next section, we elaborate on how to use this idea to decide which threshold $\epsilon_J$ should be used on the sample, assuming that the desired threshold for the database is $\epsilon$.

\usetikzlibrary{patterns}

\begin{figure*}[t!]
    \centering
\begin{tikzpicture}
\begin{axis}[%tax
    ybar,
    ymax=6000,
    enlargelimits=0.15,
    %legend style={at={(0.35,0.97)},
    %  anchor=north},
    ylabel={Runtime (seconds)},
    %xlabel={Sample size},
    %symbolic x coords={20\%,40\%,60\%,80\%,100\%},
    xtick={0,1,2,3,4},
    xticklabels={0.2,0.4,0.6,0.8,1},
    bar width=0.25,
    height=0.2\textwidth,
    width=0.25\textwidth,
        tick label style={font=\small},
    label style={font=\small},
    ]
\addplot[pattern=horizontal lines] coordinates {(0,2029.13) (1,1983.41) (2,2148.56) (3,2319.32) (4,2371.52)};\label{bar-adc}
\addplot[pattern=dots] coordinates {(0,4337.47) (1,4593.73) (2,4739.63) (3,5396.65) (4,5749.11)};\label{bar-smc}
\legend{}
\end{axis}
\end{tikzpicture}
\begin{tikzpicture}
\begin{axis}[%stock
    ybar,
    ymax=240,
    enlargelimits=0.15,
    %legend style={at={(0.35,0.97)},
   %   anchor=north},
    %ylabel={Runtime (seconds)},
    %xlabel={Sample size},
    %symbolic x coords={20\%,40\%,60\%,80\%,100\%},
    xtick={0,1,2,3,4},
    xticklabels={0.2,0.4,0.6,0.8,1},
    bar width=0.25,
    height=0.2\textwidth,
    width=0.25\textwidth,
        tick label style={font=\small},
    label style={font=\small},
    ]
\addplot[pattern=horizontal lines] coordinates {(0,42.42) (1,52.31) (2,54.21) (3,66.89) (4,79.43)};
\addplot[pattern=dots] coordinates {(0,142.72) (1,173.38) (2,184.96) (3,203.63) (4,241.31)};
\legend{}
\end{axis}
\end{tikzpicture}
\begin{tikzpicture}
\begin{axis}[%hospital
    ybar,
    ymax=80,
    enlargelimits=0.15,
    %legend style={at={(0.24,0.97)},nodes={scale=0.85, transform shape},
    %  anchor=north},
    %ylabel={Runtime (seconds)},
    %xlabel={Sample size},
        %symbolic x coords={20\%,40\%,60\%,80\%,100\%},
    xtick={0,1,2,3,4},
    xticklabels={0.2,0.4,0.6,0.8,1},
    bar width=0.25,
    height=0.2\textwidth,
    width=0.25\textwidth,
        tick label style={font=\small},
    label style={font=\small},
    ]
\addplot[pattern=horizontal lines] coordinates {(0,18.32) (1,17.43) (2,20.47) (3,19.43) (4,21.52)};
\addplot[pattern=dots] coordinates {(0,45.47) (1,51.85) (2,65.59) (3,62.34) (4,74.85)};
%\legend{$\algname{ADCEnum}$,\algname{SearchMC}}
\end{axis}
\end{tikzpicture}
\begin{tikzpicture}
\begin{axis}[%adult
    ybar,
    ymax=30,
    enlargelimits=0.15,
    %legend style={at={(0.35,0.97)},
   %   anchor=north},
    %ylabel={Runtime (seconds)},
    %xlabel={Sample size},
    %xlabel={Sample size},
        %symbolic x coords={20\%,40\%,60\%,80\%,100\%},
    xtick={0,1,2,3,4},
    xticklabels={0.2,0.4,0.6,0.8,1},
    bar width=0.25,
    height=0.2\textwidth,
    width=0.25\textwidth,
        tick label style={font=\small},
    label style={font=\small},
    ]
\addplot[pattern=horizontal lines] coordinates {(0,15.37) (1,18.14) (2,17.28) (3,18.63) (4,20.82)};
\addplot[pattern=dots] coordinates {(0,23.23) (1,20.52) (2,26.99) (3,25.29) (4,29.47)};
\legend{}
\end{axis}
\end{tikzpicture}

\begin{tikzpicture}
\begin{axis}[%airport
    ybar,
    ymax=40,
    enlargelimits=0.15,
    %legend style={at={(0.35,0.97)},
   %   anchor=north},
    ylabel={Runtime (seconds)},
    xlabel={Sample size},
        %symbolic x coords={20\%,40\%,60\%,80\%,100\%},
    xtick={0,1,2,3,4},
    xticklabels={0.2,0.4,0.6,0.8,1},
    bar width=0.25,
    height=0.2\textwidth,
    width=0.25\textwidth,
        tick label style={font=\small},
    label style={font=\small},
    ]
\addplot[pattern=horizontal lines] coordinates {(0,13.07) (1,12.13) (2,13.35) (3,14.51) (4,13.64)};
\addplot[pattern=dots] coordinates {(0,27.39) (1,22.11) (2,25.49) (3,29.2) (4,31.51)};
\legend{}
\end{axis}
\end{tikzpicture}
\begin{tikzpicture}
\begin{axis}[%inspection
    ybar,
    ymax=90,
    enlargelimits=0.15,
    %legend style={at={(0.35,0.97)},
   %   anchor=north},
    %ylabel={Runtime (seconds)},
    xlabel={Sample size},
            %symbolic x coords={20\%,40\%,60\%,80\%,100\%},
    xtick={0,1,2,3,4},
    xticklabels={0.2,0.4,0.6,0.8,1},
    bar width=0.25,
    height=0.2\textwidth,
    width=0.25\textwidth,
        tick label style={font=\small},
    label style={font=\small},
    ]
\addplot[pattern=horizontal lines] coordinates {(0,47.49) (1,46.73) (2,54.99) (3,71.37) (4,86.85)};
\addplot[pattern=dots] coordinates {(0,79.5) (1,75.1) (2,83.51) (3,78.01) (4,77.88)};
\legend{}
\end{axis}
\end{tikzpicture}
\begin{tikzpicture}
\begin{axis}[%flight - missing
    ybar,
    ymax=90,
    enlargelimits=0.15,
    %legend style={at={(0.35,0.97)},
   %   anchor=north},
    %ylabel={Runtime (seconds)},
    xlabel={Sample size},
            %symbolic x coords={20\%,40\%,60\%,80\%,100\%},
    xtick={0,1,2,3,4},
    xticklabels={0.2,0.4,0.6,0.8,1},
    bar width=0.25,
    height=0.2\textwidth,
    width=0.25\textwidth,
        tick label style={font=\small},
    label style={font=\small},
    ]
\addplot[pattern=horizontal lines] coordinates {(0,47.49) (1,46.73) (2,54.99) (3,71.37) (4,86.85)};
\addplot[pattern=dots] coordinates {(0,79.5) (1,75.1) (2,83.51) (3,78.01) (4,77.88)};
\legend{}
\end{axis}
\end{tikzpicture}
\begin{tikzpicture}
\begin{axis}[%ncvoter - missing
    ybar,
    ymax=90,
    enlargelimits=0.15,
    %legend style={at={(0.35,0.97)},
   %   anchor=north},
    %ylabel={Runtime (seconds)},
    xlabel={Sample size},
            %symbolic x coords={20\%,40\%,60\%,80\%,100\%},
    xtick={0,1,2,3,4},
    xticklabels={0.2,0.4,0.6,0.8,1},
    bar width=0.25,
    height=0.2\textwidth,
    width=0.25\textwidth,
        tick label style={font=\small},
    label style={font=\small},
    ]
\addplot[pattern=horizontal lines] coordinates {(0,47.49) (1,46.73) (2,54.99) (3,71.37) (4,86.85)};
\addplot[pattern=dots] coordinates {(0,79.5) (1,75.1) (2,83.51) (3,78.01) (4,77.88)};
\legend{}
\end{axis}
\end{tikzpicture}
\vspace{-1em}
\caption{Running times in seconds of $\algname{ADCEnum}$ (\ref{bar-adc}) and $\algname{SearchMinimalCovers}$ (\ref{bar-smc}) for varying sample sizes.}
\label{fig:ADCvsAFASTDC}
  \end{figure*}
 
  
 \begin{figure}[t!]
    \centering
    \scalebox{0.9}{
\begin{tikzpicture}
\begin{axis}[%tax
    ybar=0pt,
    ymax=50000,
    %legend style={at={(0.35,0.97)},
    %  anchor=north},
    ylabel={Runtime (seconds)},
    %xlabel={Sample size},
    %symbolic x coords={20\%,40\%,60\%,80\%,100\%},
    xtick={0,1,2,3,4,5,6,7},
    xticklabels={Tax,Stock,Hospital,Food,Airport,Adult,Flight,Voter},
    bar width=0.15,
    height=0.2\textwidth,
    width=0.53\textwidth,
    ymode=log,
    log basis y={10},
    tick label style={font=\small},
    label style={font=\small},
    enlargelimits=0.1
    ]
\addplot coordinates {(0,16138.85) (1,835.86) (2,20.28) (3,1348.31) (4,120.48) (5,83.79) (6,1000) (7,1000)};\label{20_time}
\addplot coordinates {(0,28820.62) (1,1926.83) (2,27.1) (3, 1642.92) (4,223.66) (5,175.42) (6,1000) (7,1000)};\label{40_time}
\addplot coordinates {(0,40430.23) (1,2679.4) (2,28.78) (3,1763.98) (4,262.68) (5,238.72) (6,1000) (7,1000)};\label{60_time}
\addplot coordinates { (0,0) (1,3961.02) (2,34.16) (3,2109.52) (4,421.22) (5,346.09) (6,1000) (7,1000)};\label{80_time}
\addplot coordinates { (0,0) (1,5070.65) (2,41.86) (3,2529.93) (4,563.01) (5,434.48) (6,1000) (7,1000)};\label{100_time}
\legend{}
\end{axis}
\end{tikzpicture}}
\vspace{-1em}
\caption{Running times of $\algname{ADCMiner}$ for varying sample sizes---$20\%$ (\ref{20_time}), $40\%$ (\ref{40_time}), $60\%$ (\ref{60_time}), $80\%$ (\ref{80_time}), and $100\%$ (\ref{100_time}).}
\label{fig:runtime}
  \end{figure}
  
   \begin{figure}[t!]
    \centering
    \scalebox{0.9}{
\begin{tikzpicture}
\begin{axis}[%tax
    ybar=0pt,
    ymax=2500,
    %legend style={at={(0.35,0.97)},
    %  anchor=north},
    ylabel={Runtime (seconds)},
    %xlabel={Sample size},
    %symbolic x coords={20\%,40\%,60\%,80\%,100\%},
    xtick={0,1,2},
    xticklabels={Tax,Stock,Hospital,Food,Airport,Adult,Flight,Voter},
    bar width=0.15,
    height=0.2\textwidth,
    width=0.53\textwidth,
    ymode=log,
    log basis y={10},
    tick label style={font=\small},
    label style={font=\small},
    enlargelimits=0.1
    ]
\addplot coordinates {(0,2371.52) (1,23.46) (2,79.43) (3,86.85) (4,13.64) (5,20.82
) (6,1000) (7,1000)};\label{f1_time}
\addplot coordinates {(0,2238.24
) (1,20.69) (2,63.24) (3, 85.03
) (4,12.53) (5,19.82
) (6,1000) (7,1000)};\label{f2_time}
\addplot coordinates {(0,2280.20) (1,22.55) (2,82.75) (3,90.30) (4,13.27) (5,20.27) (6,1000) (7,1000)};\label{f3_time}
\legend{}
\end{axis}
\end{tikzpicture}}
\vspace{-1em}
\caption{Running times of \algname{ADCEnum} for $f_1$ (\ref{f1_time}), $f_2$ (\ref{f2_time}), and $f_3$ (\ref{f3_time}).}
\label{fig:runtime}
  \end{figure}

\subsection{Computing the Sample Threshold}
\label{sec:find}

In this section, we focus on the following problem. Given a sample $J$, a threshold $\epsilon$ and an error bound $\alpha$, find the sample threshold $\epsilon_J$ such that if $\hat{p}< \epsilon_J$ (or, equivalently, $1-\hat{p}\geq 1-\epsilon_J$) then $\Prob(1-p\geq 1-\epsilon)\geq 1-\alpha$. We use Equation \ref{eq:dist} for this task.

Using the symmetry of the normal distribution we obtain the following.
\begin{displaymath}
\Prob \bigg[p-\hat{p}\leq z_{1-2\alpha}\cdot\sqrt{\frac{\hat{p}(1-\hat{p})}{n}}\bigg]\geq 1-\alpha
\end{displaymath}

Next, we add $1$ and subtract $1$ from the expression $p-\hat{p}$ and multiply both sides of the inner inequality by $-1$. Clearly, none of these operations affects the outer inequality and we have that:
\begin{displaymath}
\Prob \bigg[(1-p)-(1-\hat{p})\geq -z_{1-2\alpha}\cdot\sqrt{\frac{\hat{p}(1-\hat{p})}{n}}\bigg]\geq 1-\alpha
\end{displaymath}

Finally, we move the term $(1-\hat{p})$ to the other side of the inner inequality to obtain the following result.
\begin{displaymath}
\Prob \bigg[(1-p)\geq (1-\hat{p})-z_{1-2\alpha}\cdot\sqrt{\frac{\hat{p}(1-\hat{p})}{n}}\bigg]\geq 1-\alpha
\end{displaymath}

Recall that our goal is to find an $\epsilon_J$ such that if $1-\hat{p}\geq 1-\epsilon_J$ then $\Prob(1-p\geq 1-\epsilon)>1-\alpha$. Therefore, all we need to do now is setting:
\begin{displaymath}
(1-\hat{p})-z_{1-2\alpha}\cdot\sqrt{\frac{\hat{p}(1-\hat{p})}{n}}\geq 1-\epsilon
\end{displaymath}

Hence, we have that:
\begin{equation}
(1-\hat{p})\geq z_{1-2\alpha}\cdot\sqrt{\frac{\hat{p}(1-\hat{p})}{n}}+(1-\epsilon)
\label{eq:eps}
\end{equation}

Consequently, whenever $1-\epsilon_J\geq z_{1-2\alpha}\cdot\sqrt{\frac{\hat{p}(1-\hat{p})}{n}}+(1-\epsilon)$, with probability at least $1-\alpha$, an approximate DC on the sample $J$ w.r.t.~the threshold $\epsilon_J$ is an approximate DC on the entire database w.r.t.~the threshold $\epsilon$.
We conclude that we can use inequality~\ref{eq:eps} as criteria for accepting or rejecting an 
ADC on the sample.







 
